Synchronous Subsequentiality and Approximations to Undecidable Problems

We introduce the class of synchronous subsequential relations, a subclass of the synchronous relations which embodies some properties of subsequential relations. If we take relations of this class as forming the possible transitions of an infinite automaton, then most decision problems (apart from membership) still remain undecidable (as they are for synchronous and subsequential rational relations), but on the positive side, they can be approximated in a meaningful way we make precise in this paper. This might make the class useful for some applications, and might serve to establish an intermediate position in the trade-off between issues of expressivity and (un)decidability.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{J. Esparza, E. Tronci (Eds.): Games, Automata,\\ 
Logics and Formal Verification 2015 (GandALF'15)\\
EPTCS 193, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.193.5}{10.4204/EPTCS.193.5}}

